Reachability in Restricted Chemical Reaction Networks

The popularity of molecular computation has given rise to several models of abstraction, one of the more recent ones being Chemical Reaction Networks (CRNs). These are equivalent to other popular computational models, such as Vector Addition Systems and Petri-Nets, and restricted versions are equivalent to Population Protocols. This paper continues the work on core \emph{reachability} questions related to Chemical Reaction Networks; given two configurations, can one reach the other according to the system's rules? With no restrictions, reachability was recently shown to be Ackermann-complete, which resolved a decades-old problem. In this work, we fully characterize monotone reachability problems based on various restrictions such as the allowed rule size, the number of rules that may create a species ($k$-source), the number of rules that may consume a species ($k$-consuming), the volume, and whether the rules have an acyclic production order (\emph{feed-forward}). We show PSPACE-completeness of reachability with only bimolecular reactions in two-source and two-consuming rules. This proves hardness of reachability in a restricted form of Population Protocols. This is accomplished using new techniques within the motion planning framework. We give several important results for feed-forward CRNs, where rules are single-source or single-consuming. We show that reachability is solvable in polynomial time as long as the system does not contain special \emph{void} or \emph{autogenesis} rules. We then fully characterize all systems of this type and show that with void/autogenesis rules, or more than one source and one consuming, the problems become NP-complete. Finally, we show several interesting special cases of CRNs based on these restrictions or slight relaxations and note future significant open questions related to this taxonomy.

==> highlights.tex <==

\begin{highlights}
    \item First investigation into the complexity of CRNs based on several restrictions.
    \item Defined natural restrictions ``source'' and ``consuming'' for CRNs.
    \item First investigation into systems that contain only void/autogenesis rules.
    \item Prove reachability is PSPACE-complete for an extremely restricted system (most restrictive known).
    \item Show the reachability problem for certain types of systems are NP-hard.
    \item Prove that all Feed Forward systems are in NP (without void/autogenesis).
    \item Give a polynomial-time algorithm for any feed forward system without void/autogenesis rules.
    \item Give a polynomial-time algorithm for a restricted type of 1-source, 1-consuming systems.
    \item Prove that production in a 1-consuming system is NP-hard.
    \item Show that reachability with bimolecular void rules are in P.
\end{highlights}

==> models_table.tex <==
\begin{table}
    \centering
  \begin{tabular}{ | c | c | c | c | c | c |}
  \hline
  \multicolumn{6}{|c|}{\textbf{General CRNS}} \\
  \hline
  \emph{Cons.} & \emph{Source} & \emph{Rule Size} & \emph{Volume}& \emph{Membership} & \emph{Theorem}\\ \hline

  $\mathcal{O}(q)$ & $\mathcal{O}(q)$ & $(2, 2)$ & U/B & PSPACE-complete & \cite{Esparza2019} \\ \hline

  $2$ & $2$ & $(2, 2)$ & U/B & PSPACE-complete & Thm. \ref{thm:reachPSPACE} \\  \hline
  %$2$ & $2$ & $(2, 2)$  & $=^{CF}$ & PSPACE-homplete & Thm. \ref{thm:reachPSPACE} \\  \hline
  $2$ & $2$ & $(1, 2)$ and $(2, 1)$  & U/B & PSPACE-hard & Thm. \ref{thm:nonMonotone} \\  \hline
  %$2$ & $2$ & $(1,2)$ or $(2, 1)$ & U & NP-homplete & \\ \hline
  %$\geq 3$ & $1$ & $(2, 1)$ & U & NP-homplete & \\ \hline
  %$j$ & $k$ & $(1, 1)$ & U/B & NL-complete & Thm. \ref{thm:uni} \\ \hline
  $j$ & $k$ & $(1, 1)$ & U/B & NL-hard & Thm. \ref{thm:uni} \\ \hline
  \hline
  \multicolumn{6}{|c|}{\textbf{Feed-Forward}} \\
  \hline
  \emph{Cons.} & \emph{Source} & \emph{Rule Size} & \emph{Volume}& \emph{Membership} & \emph{Theorem}\\ \hline
  $2$ & $2$ & $(1, 2)$ or $(2, 2)$ or $(2,1)$ & U/B & NP-complete & Thm. \ref{thm:HamPath}\\ \hline
  $j$ & $1$ & No Void & U/B & P &  Thm. \ref{thm:ff-ss-nv-P} \\ \hline
  $1$ & $k$ & No Autogenesis & U/B & P &  Thm. \ref{thm:ff-sc-na-P}  \\ \hline
  $1$ & $1$ & Any & U/B & P & Cor. \ref{cor:ff-ss-sc-any-P}  \\ \hline
  \hline
  \multicolumn{6}{|c|}{\textbf{Feed-Forward with Void/Autogenesis Rules}} \\
  \hline
  \emph{Cons.} & \emph{Source} & \emph{Rule Size} & \emph{Volume}& \emph{Membership} & \emph{Theorem}\\ \hline
  $3$ & $0$ & $(3, 0)$ & U/B & NP-complete & Thm. \ref{thm:void3}\\ \hline
  %$j$ & $0$ & $(2, 0)$ & B & NP & Lem. \ref{lem:ff-na-NP} \\ \hline
  $j$ & $0$ & $(2, 0)$ & B & P (Bipartite) &  Thm. \ref{thm:void2bi}\\ \hline
  $j$ & $0$ & $(2, 0)$ & U & P & Thm. \ref{thm:void2uni} \\ \hline
  \end{tabular}
  \caption{Table of reachability results. The \emph{Volume} column indicates the input encoding of the volume, and thus U is for unary and B is for binary. Rule sizes $(a,b)$ indicates $a$ elements interact as input to produce $b$ elements as output. $q$ denotes the number of states in the Turing machine.} \label{tab:results}
\end{table} 

==> ncProd.tex <==
\section{Non-Competitive}
In this section we show that the producibility problem in Non-Competitive Feed-Forward CRNs is solvable in polynomial time. 


\begin{definition}[Non-Competitive]
The species of a Non-Competitive CRN can be divided into two subsets $X \bigcup Y$ where $X$ are the fuel and $Y$ are the catalysts. A reaction never consumes any species in $Y$. Each species in $X$ is net decreased by exactly $1$ reaction. 
\end{definition}

For a rule $R \in \Gamma$ and configuration $c$, let $\max(R, c)$ be the maximum number of times $R$ may be applied to configuration $c$ without performing any other rules. We provide two lemmas; the first starts with Feed-Forward rules performing a reaction without an increase in the maximum number of times an earlier rule can be directly applied. The second lemma states that in Non-Competitive systems applying a rule cannot decrease the max number of times another rule can be applied. We prove that the greedy algorithm of applying each rule maximally produces the target species if it is producible. 

\begin{lemma}\label{lem:ffInc}
For any Feed-Forward Rule set $\Gamma$ and configuration $c$, any two rules $R_i, R_j \in \Gamma$ for $i < j$, let $c' = c + R_j$, then $\max(R_i, c) \geq \max(R_i, c')$. 

\end{lemma}

\begin{proof}
Since the rule $R_j$ appears later in the feed-forward ordering, the products of that rule cannot appear as a reactant in $R_i$. This means applying $R_j$ to reach $c'$ cannot increase the number of times $R_i$ can be applied. 
\end{proof}

\begin{lemma}\label{lem:ncDec}
For any Non-Competitive Rule set $\Gamma$ and configuration $c$, any two rules $R_a, R_b \in \Gamma$, where $R_a \neq R_b$, let $c' = c + R_a$, then $\max(R_b, c) \leq \max(R_b, c')$
%performing $R_a$ will not decrease the maximum number of times $R_b$ can be applied. 
\end{lemma}
\begin{proof}
Since each species is only consumed in one rule, the species that are decreased in the rules $R_a$ and $R_b$ are disjoint, so performing one cannot decrease the number of times the other can be applied. 
\end{proof}


\begin{theorem}
The producibility problem in Non-Competitive Feed-Forward CRNs is solvable in polynomial time. (I need to work out the actual time. $\BO{|\Gamma|^2}$ times the cost of addition?)
\end{theorem}
\begin{proof}

% We will recursively compute each $\max(R_i, c)$ for $0 < i < |\Gamma|$ and storing the results in a table. 
At a high level, this algorithm goes through the feed-forward ordering, greedily performing each rule. We use the lemmas above to show correctness. At each rule, we check if we have produced the target species. If we reach a rule that consumes the target, we stop rejecting it if we have not yet produced it. We know that any rule beyond this point cannot produce the target species from the Feed-Forward restriction. 

Assuming a solution exists, we can perform some reaction $R_t$, which produces the target species. From Lemma \ref{lem:ncDec}, we know that performing any other rule cannot decrease the number of times we apply $R_t$. 

We start with the top rule $R_0$ in the feed-forward ordering.

%By Lemma \ref{lem:ffInc} performing any other rule to reach a different configuration does not increase the number of times $R_0$ can be applied. Perform $R_0$ the maximum number of times on $c$ to reach configuration $c_1$. 

Assume we have applied rules $R_0 ... R_{i_1}$ the maximum number of times and have now reached configuration $c_i$. By Lemma \ref{lem:ncDec}, we know that any rule we had previously applied doesn't decrease the maximum number of times we can apply the current rule $R_i$. So we may continue by applying $R_i$ the maximum number of times. 
\end{proof}


==> openProblems.tex <==

\subsection{Open Problems for Reachability}
For a complete characterization of reachability for all parameters, here we note the open problems and future directions of investigations.

\begin{itemize}
	\item Reachability for 1-consuming \emph{and} 1-source CRNs with the feed-forward property has membership in P. Is the feed-forward restriction required for this result or does it hold for a 1-consuming and 1-source proper CRN as well?

	\item We show the problem of reachability is PSPACE-complete with rules of size $(2,2)$.  Is reachability also hard with smaller rule sizes? Can we achieve the same result with $(2,1)$ rules and a binary encoded volume? Or is our result tight?
	
	\item Production with $(1,1)$ rules is NL-complete. However, we do not know if reachability is easy as well. Is there a polynomial time algorithm to decide unimolecular reactions?
	
	\item With a non-monotone volume we no longer have membership in PSPACE. In fact, we only have an Ackermann upper bound. With constant rule size, is reachability still Ackermann-hard?
	
   	\item Reachability for $(2,0)$ rules with the volume encoded in binary is an open problem. This is a generalized matching problem on a weighted graph. We know the problem is in $P$ for bipartite CRNs or with unary volume. Is the problem still easy in the general case?

   % \item Reachability for $(2,1)$ rules is open. For $(2,2)$ rules, we have multiple PSPACE-complete results. For $(1,1)$, we have NL-completeness. Note that $(2,1)$ rules decrease volume, so a PSPACE-complete result would need to leverage an exponential volume, something none of our current PSPACE-complete reductions utilize (they work even when the volume is polynomial bounded). On the other hand, if you can show $(2,1)$ rules imply membership in NP, we are done, as we already know this case to be NP-hard.

    %\item Reachability for single-consuming \emph{or} single-source, no void or autogenesis rules, and no catalysts. We currently know nothing about the complexity of reachability for this scenario. If any of these restrictions are relaxed, I believe we have results proving hardness.



    %\item Work out details of feed-forward membership in NP.

    %\item Exact Production Problem
        %\begin{itemize}
            %\item feed-forward, 1-consuming, no void/autogenesis, no catalysts are NP-hard for this problem, which is interesting since reachability in this scenario is in P, but the hardness uses large (exponential size) rules. What is the complexity of exact production for smaller rules (e.g., polynomial bounded)?

            %\item feed-forward, 1-source, no void/autogenesis, no catalysts are NP-hard for the same reason as above, but involves \emph{decreasing} the target species count from the initial configuration. Is exact production still hard if we try to \emph{increase} the target species?

        %\end{itemize}

\end{itemize}




==> sat.tex <==
% \subsubsection{Production is NP-Hard}
% Here, we state that production is NP-hard in single-consuming CRNs. We reduce from 3-SAT by creating species for the variables and clauses, as well as creating rules to assign variables and satisfy clauses. % 'state' used to be 'show', but I moved the proof lol

% \begin{restatable}{theorem}{singleConsumingNPhard}
%     Production in single-consuming CRNs is NP-hard.
% \end{restatable}

% %If we remove the feed-forward restriction, we can extend the reduction to Reachability by replacing the states used in the reduction once we have the SAT signal/species.

% %\begin{corollary}
% %Reachability in Non-Competitive Volume Decreasing CRNs is NP-Complete.
% %\end{corollary}

% %\subsection{Reachability in Feed-Forward Single-Consuming}

% %For a rule set $R$, let $\overleftarrow{R}$ be the reverse of the rules.

% %\begin{theorem}
% %For any two configurations $a,b$ and rule set $R$, if $a$ can reach $b$ using $R$, then $b$ can reach $a$ using $\overleftarrow{R}$.
% %\end{theorem}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%% 
